Bayesian Mechanism Design for Blockchain Transaction Fee Allocation

In blockchain systems, the design of transaction fee mechanisms is essential for stability and satisfaction for both miners and users. A recent work has proven the impossibility of collusion-proof mechanisms that achieve both non-zero miner revenue and Dominating-Strategy-Incentive-Compatible (DSIC) for users. However, a positive miner revenue is important in practice to motivate miners. To address this challenge, we consider a Bayesian game setting and relax the DSIC requirement for users to Bayesian-Nash-Incentive-Compatibility (BNIC). In particular, we propose an auxiliary mechanism method that makes connections between BNIC and DSIC mechanisms. With the auxiliary mechanism method, we design a transaction fee mechanism (TFM) based on the multinomial logit (MNL) choice model, and prove that the TFM has both BNIC and collusion-proof properties with an asymptotic constant-factor approximation of optimal miner revenue for i.i.d. bounded valuations. Our result breaks the zero-revenue barrier while preserving truthfulness and collusion-proof properties.

==> text/burning_discussion.tex <==
\ifdefined\EnableBurning

In our mechanism, as well as many other TFMs with incentive guarantees such as EIP-1559 \citep{leonardos2021dynamical} and the paper by \cite{shi}, there exists \emph{burning} in the transaction fee, which means that part of the total transaction fee is not awarded to the miner but ``wasted'', removed from the system. While the burning makes the TFM more flexible by decoupling payments on miners' and users' sides, it indeed incurs inefficiency in the utilization of funds and should be avoided or minimized if possible. Therefore, while the burning is prevalent in the design of blockchain TFMs, we are interested in the theoretical question: \textbf{is the burning really necessary}, even with the minimal incentive (U-BNIC) and collusion-proof (1-SCP) requirements?

Here, we have a result in an interesting form. Informally, the block resource and transaction fees cannot be perfectly utilized simultaneously. In other words, under mild assumptions, TFMs that have constant block size and satisfy U-BNIC and 1-SCP properties must burn some of the collected transaction fees.



Besides, while the monotonicity of allocation means a user would not decrease her allocation if she increases her bid, in a wide scope of auction mechanisms used in practice (First-Price, Second-Price, Second-Price-With-Reserve \citep{myerson1981optimal}, EIP-1559, Burning-Second-Price in \citep{shi}, etc.), we also expect the auction to be a competition among bidders on a limited number of goods, thus when a bidder increases her bid, other bidders' allocations would not increase. Therefore, we define \emph{Competitiveness} of TFMs as:

\begin{definition}[Competitiveness]
    We call a TFM $(\a,\tilde{\p},\tilde{r})$ Competitive when $\forall b_j \ge b_{j}'$,
    \begin{align}
        a_i(b_i,b_j,\b_{-ij}) \le a_i(b_i,b_{j}',\b_{-ij}).
    \end{align}
\end{definition}

The definition of Budget Feasibility (BF) only requires the miner revenue no greater than the total transaction fees collected. If the TFM has no burning, then equality should hold. We call this case Strongly Budget Feasibility (StrongBF):

\begin{definition}[Strong Budget Feasibility]
    We call a TFM $(\a,\tilde{\p},\tilde{r})$ Strongly Budget Feasible when
    \begin{align}
        \sum_{i=1}^n a_i(b_i,\b_{-i})\cdot \tilde{p}_i(b_i,\b_{-i}) = \tilde{r}(\b).
    \end{align}
\end{definition}

With assumptions on NFL and Competitiveness, we have proven the necessity of waste in either blocksize or transaction fees for non-trivial TFMs. Formally:

\begin{theorem} \label{thm:burning}
    Any TFM $\tilde{M}=(\a,\tilde{\p},\tilde{r})$ which %has constant blocksize $k$ and 
    is U-BNIC, 1-SCP, NFL, %Competitive, 
    UIR and StrongBF has constant allocation rule and zero expected miner revenue, i.e.
        \begin{align}
        a_i(b_i,\b_{-i}) &=\frac{k}{n}, \label{eqn:burn:1}\\
        E_{\b \sim V}[\tilde{r}(\b)] &= 0.\label{eqn:burn:2} 
    \end{align}
    
\end{theorem}

The proof of Theorem~\ref{thm:burning} is deferred to Appendix~\ref{app:proof:thm:burning}.

\textbf{Interpretation.} Our theorem only requires constant allocation rule and zero \emph{expected} miner revenue, but does not require the payments $\tilde{p}(b_i,\b_{-i})$ and revenue to be always zero. This is because U-BNIC only requires \emph{expectation} properties of users' payments.

Here we construct an unrigorous example: let $\mathcal{H}_i(b_i,\b_{-i})$ be a ``hash'' function uniformly distributed in $[0,1]$, and let $\tilde{p}_i(b_i,\b_{-i}) = b_i(2\mathcal{H}_i(b_i,\b_{-i})-1)$, while all (positive or negative) payments go to the miner. Then when $n\to \infty$, each individual user on expectation pays  approximately zero, so the mechanism is ``nearly U-BNIC'', and one user changing her bid does not significantly affect the expected payments of other users, so the mechanism is ``nearly 1-SCP''. Nevertheless, whether a mechanism with non-zero payments does exist, it can still be considered trivial because the bids make no effect on allocation or payments, and the miner essentially gets nothing --- still equivalent to random drawing in the long run.

\fi

==> text/global_todo.tex <==
%\com{\checkmark: Table of performance comparison of TFMs} Done

%\com{TODO: Update burning analysis} There might be some issue on our analysis for mechanisms with non-smooth allocation function. I temporarily disabled the part for burning analysis, and it can be re-added by this macro.

%\def\EnableBurning{}

\com{TODO: Implementation of sealed bids} Moved to main text (still move to appendix!), maybe need further revision

\com{TODO: Technical: Add \MUFT{1} and \MUTD{1}} Not needed as indicated by Yuan

\com{TODO: Mechanism preview ($k=1$) in intro?} But I'm unsure where... (Maybe at the end of 3.2?)

\com{TODO: How is prior ($c_\rho$) acquired? Can illustrate like other dynamic mechanisms (e.g. EIP-1559)} Compare to Shi et al..

\com{TODO: More professional specification (interim vs ex-post)} Done

\com{TODO: More comparison with literature}

\com{TODO: Less technical details in intro} Done in 1.2

\com{TODO: Significance of positive miner revenue and disadvantage of burning} If only interim budget feasibility is required then there may be no way...

\com{TODO: Advantage of sealed bids (fairness?)} Added in Section 4

\com{TODO: Discuss about MEV and PBE implementation, as suggested by R3} A little at the beginning of page 4 but i wonder if more is needed

==> text/responses/ae.tex <==
\begin{center}
    \Large \textbf{Responses to Associate Editor (AE)}
\end{center}

We are very grateful for your constructive comments, as well as your appreciation of our paper for its contribution to the OR community. We have found the comments and suggestions
useful in improving our paper and have tried our best to address them. The following is a
point-by-point response to your report. We hope the revision
is satisfactory to you.

\begin{enumerate}
    \comm{Include a discussion comparing the proposed framework with existing mechanisms such as EIP-1559 and other recent works (e.g., Wu et al., 2023). Highlight similarities, differences, and the unique contributions of the current study in relation to these approaches.}

    \resp{Thanks for the comment. We added a general discussion of EIP-1559 in Section~\ref{sec:research_q}. For the recent work \cite{wu2023maximizing}, we added it to the comparison in Table~\ref{table:comparison} and added a detailed discussion between it and our work in Section~\ref{sec:bmd}. The discussion includes comparisons of aspects of modeling, methodologies, and incentive/revenue guarantees.}

    \added{Particularly, since EIP-1559 and the work of \citet{wu2023maximizing} are both variants of posted-price mechanisms, we added detailed discussions on posted-price mechanisms in the new Section~\ref{sec:posted:price} in Related Work.}

    \comm{Provide a clearer and more explicit discussion of the miner's revenue and utility throughout the manuscript. Ensure these concepts are introduced early and defined rigorously to aid reader comprehension.}

    \resp{Thanks for the suggestion! We added early discussions of the definition (page 3) and necessity (page 5) of the miner's revenue, and added the definition of the miner's utility in our elaboration of the utility model in Section~3.3 (page 17).}

    \comm{Expand on the methodology section to provide detailed instructions on critical components such as the variation term construction. This enhancement will clarify the complexity of the research process and improve reproducibility.}

    \resp{Thanks for your advice. We added a discussion on our intuition of the variation term's construction in Appendix~\ref{app:am:intuition}, and a reference to it before the construction in Section~\ref{sec:alg:one_size}. For the scaling parameter $h$ that is important to our design, we computed the constants and derived explicit expressions in the revised version of Theorems~\ref{thm:h:value:1}-\ref{thm:h:value:k} for easier practical application and reproduction of our mechanisms.}

    \comm{Consider incorporating empirical simulations to demonstrate the practical behavior and performance of the proposed mechanisms. This addition would strengthen the paper's applicability and provide empirical support for theoretical findings.}
    
\resp{Thanks for the suggestion. We added numerical simulations for the behavior of our mechanism for general block size $k$ (Theorem~\ref{thm:h:value:k}), and the approximate MIR property (Corrolary~\ref{cor:alm:mir}). We believe that it provides practical insights as follows:}
\color{blue}
\begin{itemize}
\item In our mechanism for block size $k$, the dependence of our scaling factor $h$ on $\lambda_0$ could look complicated. With a numerical plot in Figure~\ref{fig:thm4_plot2}, we show the function $g(\lambda_0)$, the effect of $\lambda_0$ on the scaling factor $h$, in a more intuitive way.
\item In Corrolary~\ref{cor:alm:mir}, we show that the probability that MIR is violated diminishes exponentially with $n$. With a numerical plot of Figure~\ref{fig:mir}, we show the actual behavior of the probability, indicating that the MIR would hold with overwhelming probability for practical block sizes in real-world blockchains.
\end{itemize}
\color{black}

\end{enumerate}

==> text/responses/main.tex <==
\begin{center}
    {\Large \textbf{Responses to Review Reports on OPRE-2024-03-0865}}
    
    \emph{``Bayesian Mechanism Design for Blockchain Transaction Fee Allocation''}
\end{center}

We would like to thank the Area Editor, the Associate Editor, and the three referees for their time reviewing our paper, their appreciation for the novelty and contribution of our paper, and their constructive suggestions. The comments and suggestions have been very helpful in guiding
the revision. We have tried our best to address all the comments, which led to an improved version of the
paper. In particular, we have mainly made the following changes.

\begin{enumerate}
    \item Added explanations for important concepts and related studies in the Introduction to clarify the motivations and contributions of our paper.
    \item Added detailed discussions on posted-price mechanisms, including EIP-1559, mainly in Section~\ref{sec:posted:price}. Particularly, in the discussion on previous studies on TFM design, we classified the TFMs in literature into ``auction-like'' TFMs and ``posted-price'' TFMs and discussed them separately for better organization.  
    \item Added discussions on the intuitions behind our constructions of the variation term for a better understanding of our ideas and approaches, in Appendix~\ref{app:am:intuition} with a reference to it before the construction of the basic mechanism in Section~\ref{sec:alg:one_size}.
    \item Computed the constants and derived explicit expressions of scaling factor $h$ and sybil-proof properties in Theorems~\ref{thm:h:value:1}-\ref{thm:h:value:k} for clarification and convenient practical usage of our mechanisms.
    \item Added intuitive explanations of technical results before the formal theorems for easier interpretation.
    \item Added numerical simulations on critical theoretical results for empirical understanding.
    \item Clarified the writing according to the comments and corrected the typos according to the referees' comments.
\end{enumerate}

Below, we provide the changes to the paper and the responses to the detailed comments from
the associate editor and three referees, with the original comments given in \emph{italics}.

==> text/responses/r1.tex <==
\begin{center}
    \Large \textbf{Responses to Referee 1}
\end{center}

We are very thankful for your appreciation of the contribution and novelty of our paper, as well as the constructive comments that helped us improve the paper. The following is a point-by-point response to your comments. We hope that the revision is satisfactory to you.

\textbf{Major Comments:}

\begin{enumerate}
\comm{Miner’s revenue is an important objective of the research in this paper, but its discussion is missing
both in the introduction and in the subsequent sections. Readers have to dive into proofs to figure it
out. A clearer and more explicit definition and discussion of miner’s revenue would be facilitate readers’
understanding. }

\resp{Thanks for your suggestion. We added its definition in Section~1 (page 3) more discussion of the miner revenue in Section~1.1 (page 5). Particularly, we discussed it in two aspects: a higher miner revenue can incentivize miners to actively engage in mining, and excessive burning from zero-revenue TFMs may lead to a problem of \emph{deflation} that may hinder the vitality of the blockchain ecosystem.} 

\commA{A similar problem exists in Miner’s utility.}

\resp{Thanks for pointing out the missing aspect. We added the discussion of the miner's utility in Section~3.3, page 17.}

\comm{For the variation term $T$ constructed in Section 5.2, it would be beneficial to provide detailed instructions
on the process of determining the payment difference $\theta_i$. This is important because understanding
how to design an effective admissible variation term possess the real challenge in the research.}

    \resp{Thanks for your advice. We added a discussion on our intuition of the variation term's construction in Appendix~\ref{app:am:intuition}, and a reference to it before the construction in Section~\ref{sec:alg:one_size}}.

\end{enumerate}

\textbf{Minor Comments:}

\begin{enumerate}
\comm{There seems a type (typo) in the formula at the bottom of page 14. I think it should be}
\begin{align*}
&\mathbb{E}_{\b_{-i} \sim V_{-i}}[u_i(b_i,\b_{-i};v_i)] \\
    \ge &\mathbb{E}_{\b_{-i} \sim V_{-i}}\left[u_i(b_i,\b^+_{-i};v_i) + \sum_{j=n+1}^{n+l} u_j(b_{j},\b^+_{-j};0)\right].
\end{align*}

\resp{Thanks for pointing out. After carefully checking the formula, we believe that your suggestion needs to be slighted changed as follows: }

\color{blue}
\textbf{If $b_i=v_i$, then}
\begin{align*}
&\mathbb{E}_{\b_{-i} \sim V_{-i}}[u_i(b_i,\b_{-i};v_i)] \\
    \ge &\mathbb{E}_{\b_{-i} \sim V_{-i}}\left[u_i(b_i,\b^+_{-i};v_i) + \sum_{j=n+1}^{n+l} u_j(b_{j},\b^+_{-j};0)\right].
\end{align*}

Consider a scenario in which a user originally bids a higher bid than her valuation and gets a negative utility. By submitting fake transactions with zero bids she may decrease the probability of getting confirmed and decrease her loss; however, we are mainly interested in the comparison between the utilities of Sybil attacks and honest strategies. 

We are also aware that a more desirable form is
\begin{align*}
&\mathbb{E}_{\b_{-i} \sim V_{-i}}[u_i(v_i,\b_{-i};v_i)] \\
    \ge &\mathbb{E}_{\b_{-i} \sim V_{-i}}\left[u_i(b_i,\b^+_{-i};v_i) + \sum_{j=n+1}^{n+l} u_j(b_{j},\b^+_{-j};0)\right],
\end{align*}
which prevents a \emph{combination} of untruthful bids and fake transactions instead of preventing either dishonest behavior conducted individually, but due to the complexity of rigorous proofs we resort to the current version. Intuitively, as long as the occurrence of fake bids does not reach a level that substantially affects the incentive structure, the combination of two deviations (\UUB~and \UFT) that both decrease the user's utility, even with some (slight) interference with each other, usually does not increase the user's utility.

Although the revised version is mathematically equivalent to the original version, we rewrote it in the revised paper for clarity.
\color{black}

\comm{It is suggested to present some results graphically for better clarity, for example, the relationship
between users’ amount $n$ and the value of $\exp(-c_\rho^2 n)$
of Corollary 1 can be plotted by choosing a
reasonable constant $c_\rho$.}

\resp{Thanks for the advice. We added a plot for the demonstration of Corollary~\ref{cor:alm:mir} in Figure~\ref{fig:mir}.}

\comm{The acronym “MEV” seems undefined. I guess it means Miner Extractable Value. But it is better
to explicitly inform readers.}

\resp{Thanks for the reminder. We added the definition with a citation in the first occurrence in the Introduction. Its full name can be miner-extractable-value or maximal-extractable-value in different literature, with basically the same meaning.}
\end{enumerate}


==> text/responses/r2.tex <==
\begin{center}
    \Large \textbf{Responses to Referee 2}
\end{center}

We are very thankful for your appreciation to our paper, as well as the constructive comments that helps us improve the paper. The following is a point-by-point response to your comments. We hope that the revision is satisfactory to you.

\begin{enumerate}
\comm{As the authors have mentioned in the paper, the work of Gafni and Yaish (2022) adopted
a different collusion-proof notion (OCA-proofness) and developed a different Bayesian
mechanism for OCA-proofness and U-BNIC. While the paper states that the two notions
are incomparable, a very recent work (Chung et al., 2024) shows that OCA-proofness is
implied by SCP. The authors should add this discussion in the revision of the manuscript
to provide a more comprehensive overview of the current state of research in this area.}

\resp{Thanks for pointing out the recent study. We added a detailed discussion on that work and the conceptual interpretations related to SCP and OCA-proofness in Section~2.1 based on the arguments in that paper. Concisely, SCP depicts the \emph{strategy-proofness} properties and OCA-proofness is more relevant to \emph{Parato optimality} in the scope of collusions.}

\comm{A recent work by \citet{wu2023maximizing}, also motivated to maximize miner revenue in
blockchain TFM, considered a different MPC-based setting and used quite different
techniques, while also providing interesting results on Bayesian TFM design. The authors
should include a more detailed discussion and comparison of this paper, highlighting the
similarities and differences in their approaches and findings.}

\resp{Thanks for pointing out the recent work. We added the comparison between our mechanism and the work of \citep{wu2023maximizing} in the Table~\ref{table:comparison} of Introduction, and a detailed discussion in Section~\ref{sec:posted:price}.}

\comm{Although the manuscript is primarily theoretical, the authors may consider adding some
empirical simulations to virtually demonstrate the behavior and performance of the
proposed mechanism. This addition would not only strengthen the paper's practical
implications but also provide valuable insights into the real-world applicability of the
developed framework.}

\resp{Thanks for the suggestion. We added numerical simulations for the behavior of our mechanism for general block size $k$ (Theorem~\ref{thm:h:value:k}), and the approximate MIR property (Corrolary~\ref{cor:alm:mir}). We believe that it provides practical insights as follows:}
\color{blue}
\begin{itemize}
\item In our mechanism for block size $k$, the dependence of our scaling factor $h$ on $\lambda_0$ could look complicated. With a numerical plot in Figure~\ref{fig:thm4_plot2}, we show the function $g(\lambda_0)$, the effect of $\lambda_0$ on the scaling factor $h$, in a more intuitive way.
\item In Corrolary~\ref{cor:alm:mir}, we show that the probability that MIR is violated diminishes exponentially with $n$. With a numerical plot of Figure~\ref{fig:mir}, we show the actual behavior of the probability, indicating that the MIR would hold with overwhelming probability for practical block sizes in real-world blockchains.
\end{itemize}
\color{black}
\end{enumerate}

==> text/responses/r3.tex <==
\begin{center}
    \Large \textbf{Responses to Referee 3}
\end{center}

We are thankful for your detailed comments that helps us improve the paper. We revised the paper according to your comments, mainly in the following aspects:

\color{blue}
\begin{enumerate}
    \item Added detailed discussions on posted-price mechanisms, including EIP-1559, mainly in Section~\ref{sec:posted:price}. In general, the main drawback of posted-price mechanisms is that they cannot \textbf{simultaneously} satisfy 1-SCP and have positive miner revenue, and the main motivation of our paper is to bypass this impossibility result. 
    \item Added discussions on the intuitions behind our constructions of the variation term for better understanding of our ideas and approaches.
    \item Added intuitive explanations of technical results for easier interpretation.
    \item Computed the constants and derived explicit expressions of scaling factor $h$ and sybil-proof properties in Theorems~\ref{thm:h:value:1}-\ref{thm:h:value:k} for clarification and convenient practical usage of our mechanisms.
    \item Clarified the writing according to the comments and corrected the typos.
\end{enumerate}
\color{black}

The following is a point-by-point response to your comments. We hope that the revision is satisfactory to you.


\textbf{Main questions:}

\begin{enumerate}
    \comm{Does the proposed mechanism actually achieve better revenue than posting an optimal price given users' value distributions? Theoretically, the proposed mechanism achieves constant revenue when there is one slot, as the number of users $n$ goes to infinity. The optimal posted price, however, should be able to achieve revenue close to the upper bound of the support?}

\resp{An optimal posted-price mechanism without burning can achieve better revenue than ours, but it is not 1-SCP, as you commented. If we allow burning to guarantee 1-SCP, since the allocation and payment of a user is independent to others, U-BNIC implies U-DSIC and the impossibility result shows that the miner revenue of a U-DSIC and 1-SCP posted-price TFM is zero.}

\added{Additionally, from your comments we realize that the family of posted-price mechanisms is indeed an important part of existing work in TFM design. For a clearer and more organized view, we added a Section~\ref{sec:posted:price} with a detailed discussion of posted-price mechanisms, including EIP-1559 and the work of \citet{wu2023maximizing}.}
    
    \comm{What are the actual problems if the payments to the miners do not depend on the bid profile submitted by the users? In page 5 of the paper, the authors mentioned ``a non-zero additional reward for transaction confirmation besides the static block reward would indeed incentivize the miner to create the blocks honestly, in order to earn more money in additional to the basic block reward'' but did not provide any supporting arguments.} 

    \resp{In actual blockchains, the miner's total reward consists of the \emph{block reward} and transaction fees. In the modeling of our work, if the miner revenue (from transaction fees) is zero, then the miner might not get enough incentive for mining (especially for diminishing block reward setting like Bitcoin; we added the discussion in the revision in Section~\ref{sec:research_q}); if the miner revenue is a non-zero constant, the budget feasibility constraint is violated when all users bid low.}

    \added{It is worth noting that in a different MPC-based model, as proposed by \citet{wu2023maximizing}, it is possible to design a posted-price mechanism with comparable incentive and revenue guarantees to our work. The work of \citet{wu2023maximizing} utilized a different methodology from our paper due to different model settings, and their ``posted-price'' mechanism is also non-trivial as the miner revenue also needs to be carefully designed. We added a discussion of this work to Section~\ref{sec:posted:price} in the revision.}
    
    \commA{Also, the ``posted-price'' can be dynamic as well, such as the base fee in EIP 1559.}

    \resp{We added a clarification in Section~\ref{sec:research_q} that the ``posted price'' in EIP-1559 is dynamic. In the EIP-1559 protocol, as long as there is no congestion (as expected), all collected transaction fees are ``burnt'' and the miner does not get any revenue no matter what the base fee (posted price) is, and the issue that the miner may not get enough incentive would occur.}
    
    \commA{Moreover, unlike burning ``real money'', burning some tokens in a blockchain system is not necessarily value destroying. For example, reducing the circulating supply may increase the value of the token, benefiting everyone in the ecosystem (see e.g. https://ethresear.ch/t/circulating-supply-equilibrium-for-ethereum-and-minimum-viable-issuance-during-the-proof-of-stake-era/10954).}

    \resp{Thanks for your valuable point. While the burning of tokens is not necessarily value-destroying, excessive burning may lead to a problem of \emph{deflation}. In an economic perspective, deflation could be worse than inflation in the long term because it may discourage spending and investment, as people prefer holding onto their tokens rather than using (and burning) them in transactions. This behavior can hinder economic activity within the blockchain ecosystem, making it harder to sustain a thriving community. We added the discussion in Section~\ref{sec:research_q}.}

    \comm{I understand that a posted price mechanism is not collusion proof - if no bid is above the posted price, the miner may promise a side-payment to the highest bidder if she raises her bid to reach the posted price. When the number of agents goes to infinity, though, we may simply post a price at 1/2, achieve constant revenue per slot, and reduce the probability of useful collusions of this kind to zero.} 

    \resp{In this case, the expected number of users getting confirmed is a constant fraction of all users. When the number of users goes to utility, the number of \emph{confirmed users} also goes to infinity, violating the constraint that the block size is bounded to $k$. Even if we allow infinite block size, the miner may still collude with a user with a valuation of $0.49$ to ask her to bid $0.5$ instead. Then, one more transaction is confirmed, and their total utility increases by $0.49$. Since the total number of users goes to infinity, there would be many users whose valuations are slightly below $0.5$ and the probability of useful collusions would not be low.}
    
    \commA{Besides, a posted price mechanism seem to be more robust against the miners injecting fake transactions - the authors prove that the proposed mechanisms also have this properly approximately, but this relies on carefully designing the scaling factors for the variation term and I found the result (Thm 5) quite difficult to interpret given the existence of various constants.}

    \resp{While the posted-price mechanism is indeed more robust against fake transactions, as discussed above, it is either not collusion-proof, which is \emph{a main motivation} of our study, or suffers the zero revenue disadvantage. While the recent study of \citet{wu2023maximizing} did propose a variant of posted-price mechanism that satisfies collusion-proof and has positive miner revenue in a different MPC-assisted model, its design of the miner revenue rule is also non-trivial and also needs to consider various constants; besides, the notion of 1-SCP in their mechanism is substantially weaker than ours as their mechanism only allows the miner to collude with a \emph{fixed} user while our mechanism allows the miner to collude with an \emph{arbitrary} user. Hence, it suggests that even in a wide scope of different models, it is truly a non-trivial task to design TFMs that are \textbf{simultaneously} incentive compatible, collusion-proof and Sybil-proof. The posted-price mechanism, at least by itself, is not an easy shortcut to this motivation.}

    \added{For the scaling factors, we computed explicit expressions of the $h$ in Theorems~\ref{thm:h:value:1}-\ref{thm:h:value:k} and updated in the revised paper, as you also suggested in minor comment 2.}

    \added{We added intuitive explanations before the technical result and added a discussion after the Theorem~\ref{thm:almost:mic} on page 32 in the revised paper about why the result of $o(\Delta/n)$ relative advantage is non-trivial. We hope that the revised version is easier to interpret.}

    %\textbf{\textcolor{red}{Do I need to compute the constant?}}

    \comm{I also think that the writing of the paper can be improved. I had a hard time with the amount of abbreviations. }

    \resp{Thanks for the suggestion. We revised the writing according to your other comments and added a list of abbreviations in Table~\ref{table:abbr} in the Introduction section.}

    \comm{It would be helpful if the authors can provide early on some intuitive explanation of the allocation and the payment rules. }

    \resp{In Section~\ref{sec:size1}, we introduced the general pipeline of our construction that consists of the auxiliary mechanism (soft second-price mechanism) and the variation term. The idea of soft second-price mechanism was introduced in Section~\ref{sec:size1:M}: from the impossibility of deterministic U-BNIC and 1-SCP mechanisms (we also added an intuitive explanation on this impossibility result according to your minor comment 1), we need to modify the canonical first-price auction with randomization. For the intuition in the construction of the variation term, as also suggested by Referee 1, we added a discussion in Appendix~\ref{app:am:intuition} and a reference to it in Section~\ref{sec:alg:one_size}.}

    \comm{The main results (e.g. Theorems 3 and 4) are stated in very technical manners and are quite difficult to interpret.}

    \resp{Thanks for your suggestion. We added intuitive interpretations before the formal definitions in Theorems 3 and 4.}

    \comm{As various points in the paper, the authors made claims without references or supporting arguments (more details below).}

    \resp{Thanks for your advice. We added references and/or supporting arguments as specified in corresponding comments.}
\end{enumerate}

\textbf{Minor comments and questions:}

\begin{enumerate}
    \comm{I found the use of soft max in the allocation rule quite interesting. I think it would be very helpful for the readers if some intuition can be provided for Thm 9 (Appendix B), i.e. deterministic BNIC and 1-SCP mechanisms must have zero miner revenue.} 

    \resp{Thanks for the suggestion! We added an intuitive explanation of the impossibility result in Section~\ref{subsec:determ:discussion} to improve the clarity of the manuscript.}
    
    \comm{While reading through the technical section, I found myself wondering about the following: What's the intuition behind the expression of $\tilde{r}$? What are the reasons for using these second order and 4th order terms in the submitted bids? Do we have any intuitive explanation for $c_\rho$?}

    \resp{Thanks for your advice. We added a discussion on our intuition of the variation term's construction in Appendix~\ref{app:am:intuition}, and a reference to it before the construction in Section~\ref{sec:alg:one_size}. The intuition of $c_\rho$ is the expectation of $b_j^2$ and it is used to ensure $\E_{b_{-i}} [\theta_i(b_i,\b_{-i})]=0$, as one of the constraints for the admissibility of the variation term.}
    
    \commA{Is it possible to write down the expression of $h_*$?}

    \resp{For the case of $k=1$ we computed a feasible $h_*$ to be $\frac{2c_\rho (n-1)^2}{en^3}$, and for general $k$ we also computed an explicit expression of $h_*$ (which is more complicated). We updated the Theorems~\ref{thm:h:value:1}-\ref{thm:h:value:k} accordingly in the revised paper.}

    %\added{It is worth noting that it is a loose estimation due to the complexity of tighter mathematical derivations, and the actual optimal constant in the expression of optimal $h_*$ may be  larger.}

%\textbf{\textcolor{red}{[TODO: discuss about the constants.]}}
    \comm{Regarding the definition of U-SP: I think it's helpful to clarify for the main results whether we have lower bounds on $C$ and upper bounds on $N$. I can't tell this very easily from the statement of Thm 3. If the mechanism is $(C, N)$-U-SP for very small $C$ such that $Cn < 1$ then this guarantee is moot. Maybe it would be helpful to provide some actual numbers for some very simple value distributions such as Uniform[0, 1]?}

\resp{After our theoretical analysis, for any $C\in [0,1)$, the mechanism for block size 1 is $(C,\frac{6C+5}{1-C^2})$-U-SP. It shows that a dishonest user needs to insert roughly as many fake transactions as the total number of honest transactions in order to gain utility, which is a strong guarantee. The mechanism for block size $k$ can also be shown to be $\big(C,O(\frac{1}{1-C})\big)$-U-SP in a similar way. We updated our Theorem~\ref{thm:h:value:1}-\ref{thm:h:value:k} in the revised paper.}

%\textbf{\textcolor{red}{[TODO: numerical discussion for uniform distribution]}}
    
    \comm{The bounded support assumption for valuations: do we need this for the incentive properties, or the constant revenue approximation guarantees, or both (I'm assuming both?)}
    
    \resp{It is necessary only for the constant revenue approximation guarantees, as it is used in the estimation of the $h$ in the variation term. By setting $h=0$ the mechanism becomes U-DSIC and is no longer dependent on information on users' valuation distributions. The incentive properties still hold, but the miner revenue becomes zero.}

    \added{We added this case to a future research direction in the Discussion section.}
\end{enumerate}

\textbf{Typos and other issues:}

\begin{enumerate}
    \comm{dominating-strategy-incentive-compatibility $\to$ dominant-strategy incentive compatibility. See https://en.wikipedia.org/wiki/Incentive\_compatibility}

    \resp{We fixed it in the revised manuscript.}
    
    \comm{grammatical issues in the last two lines of page 2}

    \resp{Thanks for pointing out. We fixed the grammar.}
    
    \comm{line 45 of page 3: the abbreviation "MEV" is not introduced}

    \resp{We added an explanation in Introduction (miner-extractable-value or maximal-extractable-value).}
    
    \comm{The authors mentioned ``EIP 1559 economically inefficient for the miners'' in page 4. It might be helpful to clarify what ``economically inefficient'' means and why.}
    
    \resp{Thanks for the comment. We added the explanation that it means that the miners do not get any of the transaction fees collected from users.}
    
    \comm{top of page 5: the authors explained why the proposal by Chung and Shi doesn't work but I found this difficult to understand without more context}

    \resp{We added an intuition of the parameter $\gamma$ and the argument will be more understandable. On a high level, $\gamma$ is roughly the probability that a currently unconfirmed transaction would be confirmed later, which is neither easily predictable nor constant due to the fact that transactions with different bids would have different probabilities to be confirmed.}
    
    \comm{page 5, line 33: ``in additional to''}
    
    \resp{We fixed this typo and used ``in addition to'' in the revised manucript.}

    \comm{while describing desired properties, page 7 introduced FT (fake transactions) but while stating the main theorems the authors used SP (sybil-proofness) instead}

    \resp{In the context of blockchain systems, the behavior of creating multiple identities to gain an advantage is named as ``Sybil attack'', so the resilience to Sybil attacks is called ``Sybil-proofness''. In the TFM model, the actual action of a Sybil attack is to create fake transactions (discussed in Section~3.1). Hence in the context of TFM design, ``Sybil attack'' and ``fake transactions'' can be regarded as synonyms, and the resilience to \FT~can be called as Sybil-proofness.}
    
    \comm{line 50 page 12: Superscripts for footnotes should be placed after punctuation marks}

    \resp{Thanks. We fixed it.}
    
    \comm{bottom of page 14: Why does "fake transactions" necessarily have zero values? What if the user submits the same transaction multiple times (for the case of $k = 1$ it will be confirmed at most once and the agent can get their $v$ as long as one of the transactions is confirmed?)}

    \resp{When a transaction has a non-trivial value, we usually interpret that it is not ``fake'' as the users have some incentive to have it confirmed. Repeating transactions is a marginal case that may only occur when $k=1$, as in the scenario of $k\ge 2$, which is the actual practice of real-world blockchain systems, the risk of having them both confirmed (e.g., irrevocably paying for an item twice) can be perceived to be substantially higher than confirmation. On the other hand, this type of strategy is not addressed in literature either, and we can actually show that it is impossible to prevent when $k=1$. We added the discussion after Definition~\ref{def:usp} on page 18 of the manuscript.}

    \comm{page 15: do we need (expected) since we're defining ex-post budget feasibility (i.e. ex-post typically means that the condition should hold for every bid profile?) }

    \resp{While the condition should indeed hold for every bid profile, the allocation function $a(\cdot)$ is actually the probability that a transaction is confirmed, so that the  ``ex-post'' reward $\tilde{r}(\cdot)$ is also in the sense of expectation among the random drawing of confirmed transactions. However, in implementation, we can scale the actual reward to the miner proportional to the actually collected transaction fee. To be precise, when the system gets a total payment $\mathcal{P}$, the realization of miner reward is $\tilde{r}\cdot \frac{\mathcal{P}}{\sum a_i \tilde{p}_i}$.}
    
    \added{Since our paper is based on the fractional allocation model, we remove ``(expected)'' to prevent misunderstanding.}

    

    \comm{page 15-16: the definitions of UIR, BF and NFL should include for all $b_{-i}$.}

    \resp{Thanks. We added it in the definitions.}

    \comm{Definition 7: "P and" seems redundant?}

\resp{Thanks for pointing out. We removed the redundant ``$\mathbf{p}$''.}

    \comm{page 25: missing space before ``Also'' }
    
\resp{Thanks. We fixed it.}
    \comm{page 27: missing space before ``Let''}

\resp{Thanks. We fixed it.}
\end{enumerate}

==> text/revision_response.tex <==


\def\comm#1{\item \textbf{Comment: } \emph{#1}}

\def\commA#1{\noindent \textbf{Comment: } \emph{#1}}

\def\resp#1{\noindent\added{\textbf{Response: } #1}}

\setcounter{page}{1}

\input{text/responses/main}

\newpage

\input{text/responses/ae}

\newpage

\input{text/responses/r1}

\newpage

\input{text/responses/r2}

\newpage

\input{text/responses/r3}
